A Lower Bound on the Mass of Compact Objects from Dissipative Dark Matter

We study the minimum mass of dark compact objects formed in dissipative dark-matter halos and show that the simple atomic-dark-matter model consistent with all current observations can create low-mass fragments that can evolve into compact objects forbidden by stellar astrophysics. We model the collapse of the dark halo's dense core by tracing the thermo-chemical evolution of a uniform-density volume element under two extreme assumptions for density evolution: hydrostatic equilibrium and pressure-free collapse. We then compute the opacity-limited minimum fragment mass from the minimum temperature achieved in these calculations.

==> defs.tex <==
% referencing equations, sections, etc.
\newcommand{\refeq}[1]{Eq.~(\ref{eq:#1})}          
\newcommand{\refeqs}[2]{Eqs.~(\ref{eq:#1})--(\ref{eq:#2})}          
\newcommand{\refe}[1]{(\ref{eq:#1})}          
\newcommand{\refEq}[1]{Eq.~(\ref{eq:#1})}          
\newcommand{\reffig}[1]{Fig.~\ref{fig:#1}}          
\newcommand{\reffigs}[2]{Figs.~\ref{fig:#1}--\ref{fig:#2}}          
\newcommand{\reftab}[1]{Tab.~\ref{tab:#1}}
\newcommand{\refsec}[1]{Sec.~\ref{sec:#1}}
\newcommand{\refsection}[1]{Section~\ref{sec:#1}}
\newcommand{\refsecs}[2]{Sec.~\ref{sec:#1}--\ref{sec:#2}}
\newcommand{\refapp}[1]{\ref{app:#1}}


% Journal short cuts
\def\apjl{Astrophys.\ J.\ Lett.}
\def\mnras{Mon.\ Not.\ R.\ Astron.\ Soc.}
\def\nat{Nature (London)}
\def\araa{Ann. Rev. Astron. Astrophys.}
\def\aap{Astron.\ Astrophys.}
\def\apj{Astrophys.\ J.}
\def\aj{Astron.\ J.}
\def\apjs{Astrophys.\ J. Supp.}
\def\prl{Phys.\ Rev.\ Lett.}
\def\prd{Phys.\ Rev.\ D}
\def\pl{Phys.\ Lett.}
\def\physrep{Phys. Rep.}
\def\AvAA{Adv.\ Astron.\ Astrophys.}
\def\jcap{{JCAP\ }}
\def\pasj{PASJ}

% units
\def\hmpc{\,h^{-1}\,{\rm Mpc}}
\def\hmsun{\,h^{-1}\,M_{\odot}}
\def\hmmpc{\,h\,{\rm Mpc}^{-1}}
\newcommand{\Mpch}{\,h^{-1}\,{\rm Mpc}}
\newcommand{\iMpch}{\,h\,{\rm Mpc}^{-1}}
\newcommand{\Msunh}{\,h^{-1}\,M_{\odot}}

% global shortcuts
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\vs}{\nonumber\\} 
\def\ba#1\ea{\begin{align}#1\end{align}}

% brackets
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}

\def\dd{\rm d}
\def\bPsi{{\bf\Psi}}
\def\lapl{\nabla^2}
\def\laplsq{\nabla^4}

% Wigner 3-j
\def\wigner#1#2#3#4#5#6{ \left( \begin{array}{ccc} #1 & #3 & #5
\\ #2 & #4 & #6 \\ \end{array} \right)}


% macro for referencing source of figures
\newcommand{\figsource}[1]{From~\cite{#1}.}

% linear matter power spectrum
\def\Plin{P_\text{L}}
\def\pmm{\Plin}

% large-scale stochastic amplitudes
\def\Peps{P_\eps^{\{0\}}}
\def\Plapleps{P_\eps^{\{2\}}}
\def\Beps{B_\eps^{\{0\}}}
\def\BepsL{B_{\eps^L}^{\{0\}}}
\def\Pepsepsd{P_{\eps\eps_\d}^{\{0\}}}
\def\PepsepsdL{P_{\eps^L\eps_\d^L}^{\{0\}}}

% acronym for "local-in-matter-density bias"
\newcommand{\LIMD}{LIMD\xspace}

% notation for third order operator from conv. time derivative
\def\otd{\text{td}}

% symbol for D(\tau_*) / D(\tau)
\def\Dstar{\frac{D_*}{D}}
\def\Dstarinline{D_*/D}

% average number densities
\newcommand{\avnh}{\overline{n}_h}
\newcommand{\avnhell}{\overline{n}_{h\ell}}
\newcommand{\avng}{\overline{n}_g}

% spherical collapse threshold
\newcommand{\dc}{\delta_c}

% intermediate scale (assembly bias)
\def\intscale{\text{env}}

% densities
\newcommand{\rhob}{\overline{\rho}_m}
\newcommand{\Om}{\Omega_{\rm m}}
\newcommand{\Ob}{\Omega_{\rm b}}
\newcommand{\OL}{\Omega_\Lambda}
\newcommand{\Omn}{\Omega_{\rm m0}}
\newcommand{\Obn}{\Omega_{\rm b0}}
\newcommand{\OLn}{\Omega_{\Lambda0}}


% symbol for physical (rather than comoving) mean matter density
\newcommand{\rhop}{\overline{\varrho}_m}
\newcommand{\rhopb}{\overline{\varrho}_b}

% symbols for physical (rather than comoving) galaxy density
\def\ngp{\text{n}_g}
\def\avngp{\overline{\text{n}}_g}
\def\ngptilde{\tilde{\text{n}}_g}

% Laplace operator
\def\lapl{\nabla^2}
\def\laplsq{\nabla^4}
\def\ilapl{\nabla^{-2}} % inverse Laplace

% Trace (tr)
\DeclareMathOperator{\tr}{tr}

% Transpose e.g., M^\trans
\def\trans{\top}

% real and imaginary parts
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}

% log and det
\renewcommand{\ln}{\operatorname{ln}}
\renewcommand{\det}{\operatorname{det}}

% erf and erfc
\DeclareMathOperator{\erf}{erf}
\DeclareMathOperator{\erfc}{erfc}

% convective derivative
% - with respect to \tau
\def\convD{\frac{\text{D}}{{\text{D}}\tau}}
% - inline version
\def\convDinline{{\text{D}}/{\text{D}}\tau}
% - w.r.t. \ln D
\def\convDD{\frac{\text{D}}{{\text{D}}\ln D}}

% Footnote without marker, for highlighting sections as technical
\newcommand\technote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

% text highlighting
\newcommand{\bfem}[1]{\textbf{\emph{#1}}}

% capital letters
\newcommand{\vcc}{\mathrm{C}}
\newcommand{\vii}{\mathrm{I}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\Del}{\mathcal{D}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\Mm}{\mathcal{M}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\G}{\mathcal{G}}
\renewcommand{\P}{\mathcal{P}}

% vectors
\renewcommand{\v}[1]{\bm{#1}}
\newcommand{\ve}{\bm{e}}
\newcommand{\vk}{\bm{k}}
\newcommand{\vp}{\bm{p}}
\newcommand{\vq}{\bm{q}}
\renewcommand{\vr}{\bm{r}}
\newcommand{\vu}{\bm{u}}
\newcommand{\vv}{\bm{v}}
\newcommand{\vw}{\bm{w}}
\newcommand{\vx}{\bm{x}}
\newcommand{\vy}{\bm{y}}
\newcommand{\vj}{\bm{J}}
\newcommand{\bfx}{\bm{x}}
\newcommand{\bfr}{\bm{r}}
\newcommand{\bfk}{\bm{k}}
\newcommand{\bfy}{\bm{y}}
\newcommand{\bfz}{\bm{z}}

\newcommand{\vkhat}{\hat{\v{k}}}

% greek
\newcommand{\D}{\Delta}
\newcommand{\s}{\sigma}
\renewcommand{\d}{\delta}
\renewcommand{\a}{\alpha}
\renewcommand{\o}{\omega}
\newcommand{\eps}{\varepsilon}

% Sec 2
\def\L{\Lambda}
\def\xfl{\v{x}_\text{fl}}
\def\knl{k_\text{NL}}
\newcommand{\vn}{\boldsymbol{\nabla}}

% Sec 3
\newcommand{\trho}{\tilde{\rho}_m}
\newcommand{\trhop}{\tilde{\varrho}_m}
\newcommand{\tOmn}{\tilde{\Omega}_{m0}}
\newcommand{\tOKn}{\tilde{\Omega}_{K0}}
\newcommand{\tOLn}{\tilde{\Omega}_{\Lambda0}}
\def\tt{\tilde t_{0}}

% Sec 5
\def\dell{\delta_{\ell}}
\newcommand{\Fcoll}{F_{\mathrm{coll}}}
\newcommand{\cQF}{\mathcal{Q}}

% Sec 7
\newcommand{\fnl}{f_\text{NL}}
\newcommand{\taunl}{\tau_\text{NL}}
\newcommand{\gnl}{g_\text{NL}}
\newcommand{\DeltabNG}{\Delta b_1}
\newcommand{\Fs}[1]{\mathcal{F}^{(#1)}} % shape factor
\newcommand{\Sk}{S^{(3)}}

% Sec 9
\newcommand{\chit}{\tilde{\chi}}
\newcommand{\zt}{\tilde{z}}
\def\Mag{\mathcal{M}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\zhat}{\hat{z}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\ellhat}{\hat{\ell}}
\newcommand{\vnhat}{\hat{\v{n}}}

% Sec 6
\newcommand{\vpsi}{\bm{s}}   % displacement vector
\newcommand{\grad}{\boldsymbol{\nabla}} % gradient vector
\newcommand{\veta}{{\boldsymbol\eta}}
\newcommand{\vomg}{{\boldsymbol\Omega}}
\newcommand{\vlpk}{\bm{s}_\text{pk}}
\newcommand{\vxpk}{\bm{x}_\text{pk}}
\newcommand{\vvpk}{\bm{v}_\text{pk}}
\newcommand{\vqpk}{\bm{q}_\text{pk}}
% Lagrangian peak observables
\newcommand{\npk}{n_\text{pk}}
\newcommand{\fpk}{f_\text{pk}}
\newcommand{\bnpk}{\overline{n}_\text{pk}}
\newcommand{\bnesp}{\overline{n}_\text{ESP}}
\newcommand{\dpk}{\delta_\text{pk}^L}
\newcommand{\svpk}{\sigma_{v,\text{pk}}}
\newcommand{\nesp}{n_\text{ESP}}
\newcommand{\fesp}{f_\text{ESP}}
\newcommand{\xpk}{\xi_\text{pk}^L}
\newcommand{\ppk}{P_\text{pk}^L}
% Eulerian correlations
\newcommand{\xpkE}{\xi_\text{pk}}
\newcommand{\ppkE}{P_\text{pk}}
\newcommand{\xpd}{\xi_{\text{pk},\delta}^L}

% App C
% whether to put zeros in bias transformation tables in App C, or blank
\def\Ctabzero{0}
\def\Ctabzero{}

